SmartRAG: Jointly Learn RAG-Related Tasks From the Environment Feedback

RAG systems consist of multiple modules to work together. However, these modules are usually separately trained. We argue that a system like RAG that incorporates multiple modules should be jointly optimized to achieve optimal performance. To demonstrate this, we design a specific pipeline called \textbf{SmartRAG} that includes a policy network and a retriever. The policy network can serve as 1) a decision maker that decides when to retrieve, 2) a query rewriter to generate a query most suited to the retriever, and 3) an answer generator that produces the final response with/without the observations. We then propose to jointly optimize the whole system using a reinforcement learning algorithm, with the reward designed to encourage the system to achieve the best performance with minimal retrieval cost. When jointly optimized, all the modules can be aware of how other modules are working and thus find the best way to work together as a complete system. Empirical results demonstrate that the jointly optimized SmartRAG can achieve better performance than separately optimized counterparts.

==> rebuttal.tex <==
# ICLR Rebuttal

## Reviewer 1:

Thank you so much for your insightful questions and suggestions. Below, we address your questions and concerns.

**1. There exists other works focused on the question of "when to retrieval", but in Section 4.1, only one baseline was selected for comparison.**

Thank you for your reminder and concern. We will provide a more detailed explanation of this issue:

Existing research on adaptive retrieval (when to retrieve) can be broadly categorized into two types. The first type is classifier-based methods (e.g., SKR[1], AdaptiveRAG[2]), while the second type leverages GPT-4-generated data to guide the learning of this task (e.g., Self-RAG[3], RA-ISF[4]). The results for the first category of methods have already been included in the paper. As for the second category, the results for Self-RAG are presented in the table below:

| Method   | PopQA(EM) | PopQA(F1) | AmbigNQ(EM) | AmbigNQ(F1) | HotpotQA(EM) | HotpotQA(F1) |
| -------- | --------- | --------- | ----------- | ----------- | ------------ | ------------ |
| SelfRAG* | 1.07      | 23.49     | 6.12        | 26.48       | 6.80         | 17.53        |
| SKR      | 38.71     | 42.33     | 36.58       | 46.09       | 25.59        | 35.15        |
| SmartRAG | 44.32     | 47.60     | 37.89       | 47.76       | 26.60        | 36.42        | 
    
We did not include the results of SelfRAG-like methods in the paper primarily because we believe such a comparison would be unfair and lack clear significance for the following reasons:

a. SelfRAG-like methods use Accuracy as their training and evaluation metric, where any output containing the correct answer is considered correct. In contrast, we employ stricter metrics, Exact Match (EM) and F1 Score, which require complete matching for correctness. As a result, SelfRAG performs poorly under our stricter metrics, which is also corroborated by the results of SelfRAG reported in AdaptiveRAG[2]. Therefore, such a comparison holds little relevance.

b. SelfRAG relies on GPT-4 to construct a multi-supervised dataset for SFT training, particularly with 'When to retrieve' being guided directly by GPT-4. However, we argue that 'When to retrieve' should depend solely on the model itself and the knowledge base. Retrieval should occur only when the model lacks the knowledge and the knowledge base contains relevant information, rather than being determined by GPT-4's guidance.


**2. The current baselines primarily apply process-wide optimizations, without optimizing individual modules separately.**

Thank you for your valueable point! However, Sections 4.1 to 4.3 demonstrate the advantages of our approach over separate training.

**Section 4.1:** SFT RAG can be seen as optimizing only 'How to answer.' The improvement we show over SFT RAG indicates that simultaneously training the other two tasks enhances the final results. SKR, which adds a module for determining whether retrieval is necessary on top of SFT RAG, can be viewed as optimizing 'When to retrieve' and 'How to answer' separately. Our approach outperforms SKR, demonstrating that joint training yields better performance in the 'When to retrieve' task.

**Section 4.2:** In Table 4, 'Replace Query' refers to the result where the 'What to retrieve' functionality is removed. This means only 'When to retrieve' and 'How to answer' are jointly trained. The results show that the 'What to retrieve' task in SmartRAG's joint training significantly improves the outcome.

**Section 4.3:** In Table 4, 'Replace Generator' refers to the result where the 'How to answer' functionality is removed. This equates to jointly training only 'When to retrieve' and 'What to retrieve.' The results demonstrate that the 'How to answer' task in SmartRAG's joint training contributes significantly to the improvement.

**3. Discussion on the potential latency, computational overhead and training time will be benefical.**

Thank you so much for your suggestions!

**Evaluation Cost:** After training, the model produced by our approach is no different from the one following SFT in terms of inference. The inference cost per question remains the same. However, since our method reduces the retrieval percentage, we are able to decrease the average retrieval cost. The Bing API incurs a slight time cost of just over 1 second per query.

**Training Cost:** Since our method is based on RL, which inherently involves additional computational steps compared to SFT, the training cost is somewhat higher. Nevertheless, given that the training is a one-time process, this joint training approach is highly meaningful as it leads to improved training outcomes.

**4.  Considering the potential for optimizing PPO's efficiency or exploring alternative RL algorithms to reduce training costs.**

We sincerely appreciate your suggestions!

**Different RL States:** In Section 4.4 of the paper, we discuss the impact of different RL initial states on model training outcomes. The results show that a better RL initial state leads to improved model performance.

Moreover, the main focus of this paper is to demonstrate that the joint training paradigm using RL yields better results than not using RL. In future work, we will further investigate the impact of various RL methods on the overall training results of the framework.

[1] Wang, Yile, et al. "Self-Knowledge Guided Retrieval Augmentation for Large Language Models." Findings of the Association for Computational Linguistics: EMNLP 2023. 2023.
[2] Jeong, Soyeong, et al. "Adaptive-RAG: Learning to Adapt Retrieval-Augmented Large Language Models through Question Complexity." Proceedings of the 2024 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (Volume 1: Long Papers). 2024.
[3] Asai, Akari, et al. "Self-RAG: Learning to Retrieve, Generate, and Critique through Self-Reflection." The Twelfth International Conference on Learning Representations.
[4] Liu, Yanming, et al. "RA-ISF: Learning to Answer and Understand from Retrieval Augmentation via Iterative Self-Feedback." arXiv preprint arXiv:2403.06840 (2024).

We will incorporate your suggestions on these aspects in our final version. If you have any further questions or feedback, we would greatly appreciate it. We also hope this response addresses your concerns to some extent and encourages you to consider improving your final rating score, for which we would be sincerely grateful.

## Reviewer 2:

We greatly appreciate the insightful questions raised by the reviewer，which we address below and are encouraged to hear that the authors do a good job.

**1. The proposed method is very domain specific and requires the training of the entire module for each dataset.**

We deeply appreciate your concerns. We argue that any fine-tuning is specific to a particular domain, and our approach can be extended to various other domains. In the case of RAG scenarios, most current research requiring training also necessitates fine-tuning tailored to specific contexts.

**2. The generalizability of the approach is further curtailed by the availability of datasets with true final answers. (Which is needed for SFT and PPO)**

We greatly appreciate you pointing this out. Similarly, since all SFT methods rely on a golden output, this actually represents an advantage for our approach. We only rely on a single golden answer to learn three tasks, using fewer golden instances. For example, Self-RAG depends on supervisory signals generated by GPT-4 to determine whether a question requires retrieval. In contrast, we do not have any direct supervisory signals for learning 'when to retrieve' and 'what to retrieve.' The optimization of these two tasks is guided solely by the final golden answer. Therefore, we utilize fewer supervisory signals.

At the same time, if you are referring to how our framework can be applied in scenarios without a unique annotated answer, such as Dialogue, we believe that evaluation metrics commonly used in Dialogue settings, such as ROUGE, BLEU, or Consistency, could similarly be employed to compute the reward.

**3. The end to end framework requires complete retraining if any part of the framework is changed.**

Thank you for highlighting this issue!

In a multi-task collaborative framework, different components should be designed to perceive and adapt to the interactions and dependencies of other modules during their collaborative operation. In contrast, a separate training framework often optimizes submodules independently, which may lead to suboptimal solutions. Optimizing a single module assumes that different modules can collaborate seamlessly, which is not always the case.

Our joint training approach offers the following advantages:
**a. Parameter Sharing:** Joint training enhances the synergy between different parts of the model by sharing parameters, thereby improving overall performance.
**b. Avoiding Local Optima:** Joint training helps mitigate the risk of local optima that may arise from independent optimization of submodules.
**c. Reducing Error Propagation:** With a unified optimization objective, joint training minimizes error propagation between submodules, leading to improved overall performance.
**d. Resource Efficiency:** By utilizing a single LLM to address all tasks, our approach reduces the number of required modules, thereby lowering the computational cost during inference.

**4. Was all of the training data used for SFT and PPO?**

Yes, we used the same training data for both the SFT and PPO processes, with detailed data provided in Appendix A1. Specifically, for the HotpotQA dataset, in order to ensure a comparable scale to the PopQA and AmbigNQ datasets, we only used 20k training examples from HotpotQA.


**5. On which dataset was the EM and F1 evaluations done? Was this used as a part of the SFT or PPO process?**

**SFT Warm Up Stage**: In the SFT process, our goal is to train the LLM to produce outputs for different tasks. The overall training procedure follows a structure similar to other SFT processes. Here, EM and F1 metrics were not employed; instead, we fine-tuned the LLM using traditional Cross Entropy Loss. The input consists of a question along with a template (as shown in Appendix Table 7), and the output is either [Answer] or [Retrieve].

**RL Training Stage**: In the RL training process, the end marker for each training example is the response [Answer]. For each output sentence, there are two possible types of actions: [Answer] and [Retrieve]. Each action at every step of the RL process is assigned a reward score (or 0). We set the reward for [Retrieve] to -0.2, while the reward for [Answer] is based on the accuracy of the answer, calculated using EM and F1. The more accurate the answer, the higher the [Answer] reward. EM and F1 are also the evaluation metrics we use to assess the quality of the model's responses, and they are among the most commonly used evaluation metrics in QA scenarios.

During the RL process, we calculate EM and F1 for the output of each training example in the dataset to compute the reward, which means that these metrics need to be evaluated for all the entire training set. Similarly, when assessing the model's performance, we also calculate the EM and F1 scores for the outputs of the test set, which serve as the final evaluation results.

**6. Is SFT RAG the performance of \Phi_\theta in the setting described in Figure 1? (Was SFT RAG evaluated in the same setting as SmartRAG? where the policy network was allowed one retrieval? )**

SFT RAG is trained using data that includes only answers after retrieval, resulting in a setup consistent with the SFT warm-up phase before RL initialization. However, the training data differs slightly, as it does not involve the 'what to retrieve' and 'direct answer' tasks.

Both SFT RAG and SmartRAG use the same evaluation settings, with a maximum retrieval limit of 1 during both training and testing. As mentioned in line 251, we set the retrieval quota to 1.


**7. Have the authors tried using the weaker LLM to generate the SFT query dataset?****

Thank you very much for your valuable suggestions!

We further replaced GPT-3.5 with LlaMA2-7B to generate our query dataset, while keeping all other settings unchanged. The results on Flan-T5-large are as follows:

| Query Generator | PopQA(EM) | PopQA(F1) | AmbigNQ(EM) | AmbigNQ(F1) | HotpotQA(EM) | HotpotQA(F1) |
| --------------- | --------- | --------- | ----------- | ----------- | ------------ | ------------ |
| LlaMa2-7B       | 42.22     | 45.97     | 34.33       | 43.88       | 25.33        | 35.32        |
| GPT35           | 42.50     | 45.95     | 33.71       | 42.75       | 25.54        | 35.23        |
    
It can be observed that using different Query Generators has minimal impact on the overall results; in fact, LLaMA2-7B achieves better performance on the AmbigNQ dataset. This is because the Query Dataset serves only as an initialization for query learning, rather than representing an optimal state. The significantly better performance of SmartRAG compared to GPT-4 Rewriter + SFT RAG further supports this point: 'What to retrieve' should not be determined by GPTs but should instead be jointly decided by the LLM itself and the knowledge base. Our joint training framework enables query generation to take both the knowledge base and the LLM into account, thus achieving superior results.

Finally, we sincerely thank you for your efforts. If our response has addressed your concerns to some extent, we would greatly appreciate your positive consideration in the rating score. Your support would mean a lot to us！

## Reviewer 3:

We greatly appreciate your feedback and questions. Below are our explanations for some of the issues you raised:

**1. Why does the policy network serve three roles in the model? What's the motivation behind it? Won't these three roles conflict with each other?**

a. Multitask Capability of LLMs: LLMs inherently possess the ability to solve multiple tasks simultaneously, which is one of their significant advantages. Therefore, we aim to leverage this capability to optimize several RAG-related tasks concurrently, relying solely on environment feedback.

b. Conflicts Between Different Tasks: Conflicts may arise between different tasks; however, this is not the main focus of our study. Our primary concern is the final outcome, and task conflicts are viewed as an intermediate challenge, dependent on the model's compatibility across tasks. Our experimental results demonstrate that SmartRAG effectively improves performance on three key tasks: when to retrieve, what to retrieve, and how to answer.

Finally, similar to instruction tuning, where optimizing multiple tasks simultaneously may lead to task conflicts, addressing multiple tasks with a single model remains highly meaningful.


**2. How to distinguish whether a low reward is caused by a wrong policy or inaccurate retrieval?**

Thank you for noticing this detail—it is indeed a crucial aspect of our paper!

The [Retrieve] action is penalized with −α, where 
�� = 0.2. Following retrieval, there are two possible outcomes:

**a. Correct Answer After Retrieval:** If the subsequent [Answer] is correct, it receives a reward of +2. In this case, the value of the state after [Retrieve] becomes 2×Decay−0.2, where Decay is the reward decay factor, a number close to 1. This makes the value of the state after [Retrieve] (given a correct answer) a significantly positive number.

**b. Incorrect Answer After Retrieval:** If the subsequent [Answer] is incorrect, it receives a reward of 0. Here, the value of the state after [Retrieve] becomes −0.2.

Without retrieval, there are two possible outcomes:
 
**c. Correct Answer without Retrieval:** Since no retrieval penalty is incurred, the total reward in this case is simply the reward from the [Answer], which equals +2.

**d. Incorrect Answer without Retrieval:** Since no retrieval penalty is incurred, the total reward in this case is simply the reward from the [Answer], which equals 0.

The LLM's policy decisions are primarily based on value estimation. The values of the four possible states are ranked as: c > a > d > b. Therefore, the model will prioritize answering correctly and then consider the necessity of retrieval. This prioritization enables SmartRAG to simultaneously reduce the retrieval percentage while enhancing final performance.

If your question concerns whether an incorrect final [Answer] results from a model error or an incorrect retrieval, we address this as follows:

**From a Training Perspective:** Both types of errors can potentially lead to an incorrect [Answer]. However, the model’s policy actively explores ways to optimize its behavior. On the one hand, it refines the query to retrieve more relevant information; on the other hand, it adjusts its [Answer] output to generate more accurate content. During training, we do not need to explicitly distinguish between these two types of errors, as reinforcement learning (RL) aims to explore and optimize a more accurate policy overall.

**From an Evaluation Perspective:** In QA tasks, the relevance of the retrieved content is a key evaluation metric. The "hit" metric in Table 4 indicates the proportion of retrieved content that contains the correct answer. We can consider retrieval errors as instances where there is no "hit," in which case the retrieval itself is deemed faulty. If the retrieval is correct but the final answer is wrong, we attribute the error to the model's own decision-making rather than to an issue with retrieval.


**3. Why is the retrieval percentage of SKR in Figure 2 fixed at 0.8?**

Since SKR is based on a classifier approach, methods based on classifiers or clustering can ultimately produce only a deterministic result—either retrieval or no retrieval. In contrast, SmartRAG adjusts the retrieval confidence threshold, allowing for a range of retrieval percentages, rather than a fixed decision.


**4. Why does SFT RAG yield the best performance in 2 out of 3 cases with the highest retrieval ratio? Which is conflcit to the statements.**

Thank you for pointing that out. What we meant in the original text is that we believe Bing struggles to retrieve useful information from the OpenBookQA, MedQA-cn, and ARC-c datasets, rather than being completely unable to retrieve anything. From the results, we observe that SFT RAG only outperforms SFT by about one point on average, suggesting that in approximately 99% of cases, RAG fails to retrieve relevant content in these datasets. Therefore, in such scenarios, we argue that RAG is not necessary.

**5. The RAG baselines seem not extensive, compared with references on this topic.**


Thank you very much for your reminder and concern. We will provide a more detailed explanation of this issue:

Existing research on adaptive retrieval (when to retrieve) can be broadly categorized into two types. The first type is classifier-based methods (e.g., SKR[1], AdaptiveRAG[2]), while the second type leverages GPT-4-generated data to guide the learning of this task (e.g., Self-RAG[3], RA-ISF[4]). The results for the first category of methods have already been included in the paper. As for the second category, the results for Self-RAG are presented in the table below:

| Method   | PopQA(EM) | PopQA(F1) | AmbigNQ(EM) | AmbigNQ(F1) | HotpotQA(EM) | HotpotQA(F1) |
| -------- | --------- | --------- | ----------- | ----------- | ------------ | ------------ |
| SelfRAG* | 1.07      | 23.49     | 6.12        | 26.48       | 6.80         | 17.53        |
| SKR      | 38.71     | 42.33     | 36.58       | 46.09       | 25.59        | 35.15        |
| SmartRAG | 44.32     | 47.60     | 37.89       | 47.76       | 26.60        | 36.42        | 
    
We did not include the results of SelfRAG-like methods in the paper primarily because we believe such a comparison would be unfair and lack clear significance for the following reasons:

a. SelfRAG-like methods use Accuracy as their training and evaluation metric, where any output containing the correct answer is considered correct. In contrast, we employ stricter metrics, Exact Match (EM) and F1 Score, which require complete matching for correctness. As a result, SelfRAG performs poorly under our stricter metrics, which is also corroborated by the results of SelfRAG reported in AdaptiveRAG[2]. Therefore, such a comparison holds little relevance.

b. SelfRAG relies on GPT-4 to construct a multi-supervised dataset for SFT training, particularly with 'When to retrieve' being guided directly by GPT-4. However, we argue that 'When to retrieve' should depend solely on the model itself and the knowledge base. Retrieval should occur only when the model lacks the knowledge and the knowledge base contains relevant information, rather than being determined by GPT-4's guidance.

[1] Wang, Yile, et al. "Self-Knowledge Guided Retrieval Augmentation for Large Language Models." Findings of the Association for Computational Linguistics: EMNLP 2023. 2023.
[2] Jeong, Soyeong, et al. "Adaptive-RAG: Learning to Adapt Retrieval-Augmented Large Language Models through Question Complexity." Proceedings of the 2024 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (Volume 1: Long Papers). 2024.
[3] Asai, Akari, et al. "Self-RAG: Learning to Retrieve, Generate, and Critique through Self-Reflection." The Twelfth International Conference on Learning Representations.
[4] Liu, Yanming, et al. "RA-ISF: Learning to Answer and Understand from Retrieval Augmentation via Iterative Self-Feedback." arXiv preprint arXiv:2403.06840 (2024).

Thank you so much for taking the time to review our paper and responses. We hope this response adequately addresses your concerns. If so, we sincerely hope you might consider improving your rating score, for which we would be deeply grateful!

## Reviewer 4:

We sincerely appreciate your affirmation of the ideas presented in our paper. Next, we will address and clarify some of the concerns you have raised.

**1. Why there is a pre-specified quota for retrieval？**

Thank you for highlighting the issue of retrieval cost, which is often overlooked in industrial applications. We must acknowledge that retrieval can indeed reliably enhance performance. However, the definition we propose is based on following two key considerations:

**a. Retrieval cost:** The Bing retrieval module we employed in our study incurs a time cost of over 1 second per query, and other deployed open-domain knowledge retrieval modules generally exceed this cost. We believe it is meaningful to reduce this cost to some extent while maintaining or even improving performance. This aligns with the motivation behind several existing adaptive retrieval studies. While we agree with your perspective that a solid answer is more critical than retrieval cost, we argue that balancing both factors offers greater practical significance.

**b. This is just a experimental setting:** In our study, we set the retrieval quota to 1 to ensure a fair comparison with existing methods. Current methods such as SFT RAG and other single-retrieval approaches (except Multi-Step RAG) typically perform only a single retrieval. To demonstrate that our improvements are not derived from multiple retrievals, we adopted this setting to ensure fairness. Of course, in practical applications, you could set a larger retrieval quota or even remove it entirely, as the quota is not a mandatory constraint.

We hope this clarifies and resolves your concerns regarding the motivation behind this specific setting.

**2. The optimization seems not fully end-to-end.**

Thank you for pointing out that the knowledge base itself, as well as the matching mechanism between knowledge and queries, are critical components of RAG systems. 

In our framework, we primarily use Bing for retrieval, largely due to its speed and efficiency. Consequently, the knowledge base in our framework is treated more as a utility tool. Our work primarily focuses on optimizing tasks related to the parameters of the LLM itself. Additionally, we have improved the query rewrite task associated with knowledge retrieval. The results in Table 4 demonstrate that simply optimizing the LLM can significantly enhance the accuracy of retrieval matching.


**3. os is the concatenation of all the historical observations，how to solve the problem of LLM token limit?**

Our retrieval quota is set to 1, and the number of retrieved passages is limited to 4. As a result, the concatenated of historical observations does not encounter issues related to the LLM token limit.


**4. Why [retrieve] action suffers from a 100% penalty in equation (5) of the reward design?  how about the correct answer generated from retrieved observations?**


Thank you for noticing this detail—it is indeed a crucial aspect of our paper!

The [Retrieve] action is penalized with −α, where 
�� = 0.2. Following retrieval, there are two possible outcomes:

**a. Correct Answer After Retrieval:** If the subsequent [Answer] is correct, it receives a reward of +2. In this case, the value of the state after [Retrieve] becomes 2×Decay−0.2, where Decay is the reward decay factor, a number close to 1. This makes the value of the state after [Retrieve] (given a correct answer) a significantly positive number.

**b. Incorrect Answer After Retrieval:** If the subsequent [Answer] is incorrect, it receives a reward of 0. Here, the value of the state after [Retrieve] becomes −0.2, which is negative.

The LLM's policy decisions are primarily based on value estimation. Since retrieval followed by a correct answer leads to a relatively high state value, the model is incentivized to retrieve when it anticipates a correct answer post-retrieval.

Now, consider a case where the model can directly answer correctly without retrieval.

**c. Correct Answer without Retrieval:** Since no retrieval penalty is incurred, the total reward in this case is simply the reward from the [Answer], which equals +2.

Thus, the value of the state corresponding to directly answering correctly (+2) is higher than that of answering correctly after retrieval (2×Decay−0.2).

Under our training framework, the model prioritizes states with higher values. The hierarchy of priorities becomes: 1. Directly answering correctly. 2. Retrieving and then answering correctly. 3.Directly answering incorrectly. 4. Retrieving and then answering incorrectly. This prioritization allows SmartRAG to simultaneously reduce the retrieval percentage and enhance final performance.

Finally, we sincerely thank you for taking the time out of your busy schedule to read our paper and provide valuable feedback. If the responses above have addressed your concerns to some extent and you would consider raising your score, we would greatly appreciate it. If you have any further suggestions or questions, we warmly welcome your additional feedback!

==> sections/4experiments_bk.tex <==
\section{Experiments}
%\subsection{Implementation Details and Baselines}

\myparagraph{Dataset.} Following \citet{queryrewrite}, we use three open-domain QA datasets for evaluation, namely PopQA~\citep{mallen2023not}, AmbigNQ~\citep{min2020ambigqa} and HotpotQA~\citep{yang2018hotpotqa}. Besides, we also use other datasets like TrivialQA~\citep{joshi2017triviaqa}, OpenBookQA~\citep{openbookqa}, MedQA-cn~\citep{medqa} and ARC-c~\citep{arc} for more analysis and comparisons. All the details of the related datasets are shown in Appendix~\ref{sec:dataset}.
% Similiar to \citet{queryrewrite}, three open-domain QA datasets are used for evaluation. Additionally, we incorporate TriviaQA~\citep{joshi2017triviaqa} for dataset transfer testing. Furthermore, we introduce three multi-choice QA datasets to validate our method's ability to be aware of and effectively utilize database retrieval. Details of datasets are shown in the Appendix \ref{sec:dataset}.

\myparagraph{Retriever.} We utilize Bing search engine as our retriever $\mathcal{R}$, which offers a broad knowledge scope and ensures up-to-date factual information. The search engine will return multiple results given a query. We select the top $K$ results and concatenate the snippets from these results as the observation. We leave how to utilize these snippets for the answer generator. In our experiments, we set $K=4$ without other clarifications.
%We utilize the Bing search engine as our retriever, which does not require candidate index construction like dense retrievers, nor predefined candidates as in traditional resources. Instead, it offers a broad knowledge scope and ensures up-to-date factual information. Retrieval via the Bing API is conducted through two methods. First, we concatenate snippets from all retrieved web pages, selecting relevant sentences identified by Bing—much like entering a query into a browser, then gathering the text displayed on the search results page. Second, we request the URLs of the retrieved pages and parse the entire content, akin to clicking on individual search results. To maintain a balance between accuracy and length constraints, we set the default number of retrievals to four.

\myparagraph{Training Details.} For the SFT warmup stage, we use the following training parameters: a learning rate of $3e-4$, a batch size of $8$ and the training epochs is set to $1$ to avoid overfitting. For the reinforcement learning stage, we use an on-policy sampling strategy. For each iteration, we sample many trajectories such that the total length of all these trajectories is $5120$. The policy network is then trained for $1$ epoch on these samples with the learning rate being $2e-6$ and batch size being $32$. The retrieval penalty $\alpha$ in (\ref{reward}) is set to $0.2$ and the retrieval quota $N$ is specified to be $1$ to fairly compare with other baselines.
%We use 4 Nvidia A100 with 80GB memory to train our models. For both the warm-up and SFT phases, we used the same training parameters: a learning rate of 3e-4, a batch size of 8, and to prevent overfitting, the number of epochs is set to 1. For reinforcement learning, we set the sampling steps to 5120, 10 threads, 512 steps for each. After sampling, the policy network is trained for 1 epochs, with learning rate as 2e-6 and batch size as 32. For the retrieval reward $\alpha$ in equation \ref{reward}, we set it to 0.2. 

More implementation details are introduced in Appendix~\ref{sec:implementation}. We compare our method with the following baselines.

% \subsection{Baselines}
%To conduct a holistic evaluation and comparison,we use the same datasets, with the same retrieverand corpus to compare our method with the follow-ing baselines. We split them into two categories.

\myparagraph{Vanilla RAG} first retrieves the search engine using the input question. Then it asks the LLM to generate the final answer with the observations returned from the search engine in a few-shot manner.

\myparagraph{SFT RAG} uses the same pipeline as our SmartRAG. Similar to Vanilla RAG, it uses the input question to retrieve the search engine. We then use finetune the answer generator given the input question along with the observations. 

\myparagraph{GPT4 Rewriter + SFT RAG} adds a query rewrite module than \textbf{SFT RAG}. We ask GPT4, which is one of the most powerful LLMs, to rewrite the searching query before feeding it to the search engine. In this case, all the modules are still separately optimized.

\myparagraph{ReAct}~\citep{yao2023react} uses the inherent ability of the base network to decide how to retrieve and answer using chain-of-thought (CoT)~\citep{wei2022chain}. It can also self reflect the previous queries and answers to arrive at the final answer, with the hint from the golden answer. 

\myparagraph{IRCoT}~\citep{trivedi2023interleaving} enhances each step of the CoT generation process by incorporating knowledge retrieval steps during the generation process. Note that both ReAct and IRCoT uses multi-step retrieval such that the retrieval cost is higher than other baselines and our SmartRAG.

% \myparagraph{SKR}~\citep{wang2023self} trains a small model to determine whether the LLM can answer a question using its own knowledge.

%\myparagraph{Baselines with retrieval.} \textbf{Direct RAG} is similar to ICL, while using retrieval augmentation on cases and generation. \textbf{SFT RAG} is full answer from retrieval after self-instruction tuning. \textbf{ReAct}~\citep{yao2023react} is that enables the model to self-reflect on when to retrieve information and how to formulate the retrieval query. By iteratively refining the query and reflecting on the answer, it guides the model towards arriving at the final answer. \textbf{IRCoT}~\citep{trivedi2023interleaving} enhances each step of the chain-of-thought generation process by incorporating knowledge retrieval steps during the generation process. Both ReAct and IRCoT are mult-step retrieval. \textbf{SKR}~\citep{wang2023self} trains a small model to determine whether the LLM can answer a question using its knowledge and decides whether to perform retrieval for the given question.

%\myparagraph{Baselines without retrieval.} \textbf{ICL} employed the in-context learning approach by providing the original LLM with two examples and straightforward instructions to follow. \textbf{SFT} is directly answer evaluation after self-instruction tuning.

All the above baselines use at least one time of retrieve. To further show the baseline without any retrieval, we also compare with two extra baselines, namely \textbf{ICL} which is a few-shot inference, and \textbf{SFT} which is directly finetuned on the golden answer.

\begin{table*}
    \centering
    \footnotesize
    \resizebox{0.98\textwidth}{!}{
    
        \begin{tabular}{lcccccccc}
            \toprule
            {\multirow{2}{*}{\textbf{Model}}}  & \multicolumn{2}{c}{\textbf{PopQA}}  & \multicolumn{2}{c}{\textbf{AmbigNQ}} &  \multicolumn{2}{c}{\textbf{HotpotQA}} &  \multicolumn{2}{c}{\textbf{Average}}  \\
            \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-9}
            & \textbf{Exact Match} & \textbf{F1} & \textbf{Exact Match} & \textbf{F1} & \textbf{Exact Match} & \textbf{F1} & \textbf{Exact Match} & \textbf{F1} \\
            \midrule
            % \multicolumn{8}{c}{\textbf{\textit{Flan-T5 base Without Retrieval}}} \\
            %  ICL &  7.01 &  9.10 & 1.37  & 5.40 &  9.85 & 15.43  &    \\
            %  SFT & 11.78 & 16.64 & 2.39 & 7.80  &  11.23  & 17.71  &    \\
            %  SFT-S & 12.48 & 17.13 & 2.53 & 8.20 & 11.28 & 18.18 &   \\
            % \midrule
             
            % \multicolumn{8}{c}{\textbf{\textit{Flan-T5 base With Retrieval}}} \\
            % Direct RAG & 23.14 & 26.77  &  15.68 & 24.48 &  15.83 &  23.94 &    \\
            % SFT RAG & 30.72 & 35.35 & 16.96 & 25.92  &  17.68 &  26.13 &    \\
            % SFT RAG-S &  &  &  &   &   &  &    \\
            % SKR\textsubscript{knn}~\citep{SKR} & 23.98 &  28.08 &  16.60 & 25.40 & 16.98  &  25.23 &    \\
            % Ours & 33.66 & 37.87 & 18.31  & 27.71 & 18.24  &  27.26 &    \\
            % \midrule
            % \multicolumn{8}{c}{\textbf{\textit{Flan-T5 large Without Retrieval}}} \\
            %  ICL &  7.03 & 10.16 &  2.47 & 7.30 &  12.46 & 20.42 & \\
            %  SFT & 12.62 & 17.79 & 3.86 &  10.12 & 12.60 &  19.41 &  \\
            %  SFT-S & 12.76 & 17.70 & 4.56 &  10.92 & 13.62 & 20.74 &  \\
            % \midrule
            % \multicolumn{8}{c}{\textbf{\textit{Flan-T5 large With Retrieval}}} \\
            % Direct RAG & 28.34 & 32.79 & 19.88 & 29.53 & 17.96 & 28.12 &  \\
            % SFT RAG  & 32.82 & 37.06 & 20.11 & 30.45 & 20.83 & 30.01 &\\
            
            % SFT RAG -S  & 32.11 & 36.13 & 18.83 & 29.05 & 19.89 & 29.58\\
            % % SKR\textsubscript{knn}~\citep{SKR}  & 33.38 & 37.15 & 26.83 & 35.97 & 23.5 & 32.41 & \\
            % SKR\textsubscript{knn}~\citep{SKR}  & 28.56 & 32.35 & 17.11 & 26.96 &  19.36 & 27.96 & \\

            % Ours & 35.48 & 39.73 & 20.53 & 30.94 & 22.17 & 31.72 &\\
            \multicolumn{9}{c}{\textbf{\textit{Flan-T5 large Without Retrieval}}} \\
             ICL &  7.03 & 10.16 &  2.47 & 7.30 &  12.46 & 20.42 & 7.32 & 12.63 \\
             % SFT & 12.62 & 17.79 & 3.86 &  10.12 & 12.60 &  19.41 &  \\
             % SFT-S & 12.76 & 17.70 & 4.56 &  10.92 & 13.62 & 20.74 &  \\
             SFT & 12.76 & 17.70 & 4.56 &  10.92 & 12.72 & 19.72 & 10.01 & 16.11  \\
            \midrule
            \multicolumn{9}{c}{\textbf{\textit{Flan-T5 large With Retrieval}}} \\
            Vanilla RAG & 34.36 & 38.80 & 30.72 & 40.16 & 22.06 & 32.57 &  29.05 & 37.18 \\
            % SFT RAG  & 32.82 & 37.06 & 20.11 & 30.45 & 20.83 & 30.01 &\\
            SFT RAG & 38.15 & 42.05 &  31.63 & 41.05 & 24.01 & 34.03 & 30.93 & 38.68 \\
            GPT4 Rewriter + SFT RAG & \underline{39.27} & \underline{42.68} & \underline{33.43} & \underline{42.40} & \underline{24.12} & \underline{34.33} & \underline{32.27} &  \underline{39.80} \\
            SKR\textsubscript{knn}~\citep{SKR}  & 33.38 & 37.15 & 26.83 & 35.97 & 22.32 & 31.39 & 27.51 & 34.84 \\
            % SKR\textsubscript{knn}~\citep{SKR}  & 28.56 & 32.35 & 17.11 & 26.96 &  19.36 & 27.96 & \\

            % Ours & 41.66 & 45.95 & 32.68 & 42.56 & 26.08 & 36.26 &\\
            \textbf{SmartRAG(ours)} & \textbf{42.50} & \textbf{45.95} & \textbf{33.71} & \textbf{42.75} & \textbf{25.54} & \textbf{35.23} & \textbf{33.29} & \textbf{41.25} \\
            \midrule
            % \multicolumn{8}{c}{\textbf{\textit{Flan-T5 XL Without Retrieval}}} \\
            %  SFT  & 15.43 & 19.77 & 5.83 & 12.49 & 14.10 & 20.99 &\\
            % \midrule
             
            % \multicolumn{8}{c}{\textbf{\textit{Flan-T5 XL With Retrieval}}} \\
            % SFT RAG & 34.64 & 38.93 &  &  &  & &\\
            % SKR\textsubscript{knn}~\citep{SKR}  & & & & & & &\\
            % Ours & & & & & & &\\
            % \midrule
            % \multicolumn{8}{c}{\textbf{\textit{LlaMa-2 7B Without Retrieval}}} \\
            % % Direct & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
            % % CoT &  &  &  &  &  &  &  \\
            % ICL & 21.79 & 24.61 & 18.63 & 27.12 & 17.62 & 25.60 &  \\
            % SFT & 25.81 & 30.39 & 22.03 & 31.24 & 19.72 & 28.24 & \\
            
            % % Least-to-most &  &  &  &  &  &  &   \\
            % \midrule
            % \multicolumn{8}{c}{\textbf{\textit{LlaMa-2 7B With Retrieval}}} \\
            % Direct RAG & 28.91 & 34.94 & 28.05 & 36.85 & 25.15 & 35.87 &  \\
            % SFT RAG & 37.17 & 40.33 & 28.43 & 38.42 & 25.59 & 35.32 &  \\
            % ReAct~\citep{yao2023react} & 27.21 & 31.49 & 22.45 & 31.24 & 21.91 & 29.83 &   \\

            % IRCoT~\citep{trivedi2023interleaving} & 9.22 &  17.93 & 13.52 & 25.94 & 17.42 & 27.13 &  \\
            % SKR\textsubscript{knn}~\citep{SKR} & 34.01 & 37.56 & 27.30 & 36.11 & 24.17 & 33.61 &   \\
            % Ours & 38.38 & 41.19 & 32.19 & 41.28 & 25.99 & 36.84 &   \\
            % \bottomrule

            % \multicolumn{9}{c}{\textbf{\textit{LlaMa-2 7B Without Retrieval}}} \\
            % ICL & 21.79 & 24.61 & 18.63 & 27.12 & 17.62 & 25.60 & 24.23 & \\
            % SFT & 27.91 & 31.54 & 22.47 & 31.28 & 20.74 & 29.52 & 27.24 &  \\
            % \midrule
            % \multicolumn{8}{c}{\textbf{\textit{LlaMa-2 7B With Retrieval}}} \\
            % Direct RAG & 33.38 & 40.37 & 30.91 & 42.77 & 25.15 & 35.87 & 34.74 & \\
            % SFT RAG & \underline{42.92} & \underline{46.60} & \underline{30.50} & \underline{41.02} & \underline{25.59} & \underline{35.32} & \underline{36.99} & \\
            % ReAct~\citep{yao2023react} & 27.21 & 31.49 & 22.45 & 31.24 & 21.91 & 29.83 &  27.36 & \\
            % IRCoT~\citep{trivedi2023interleaving} & 9.22 &  17.93 & 13.52 & 25.94 & 17.42 & 27.13 & 18.53 & \\
            % SKR\textsubscript{knn}~\citep{SKR} & 39.27 & 43.40 & 29.29 & 38.55 & 24.17 & 33.61 &  34.72 & \\
            % \textbf{SmartRAG(ours)} & \textbf{44.32} & \textbf{47.60} & \textbf{34.53} & \textbf{44.07} & \textbf{25.99} & \textbf{36.84} & \textbf{38.89} & \\
            \multicolumn{9}{c}{\textbf{\textit{LlaMa-2 7B Without Retrieval}}} \\
            ICL & 21.79 & 24.61 & 18.63 & 27.12 & 17.62 & 25.60 & 19.35 & 29.11 \\
            SFT & 27.91 & 31.54 & 22.47 & 31.28 & 20.74 & 29.52 & 23.71 & 30.78 \\
            \midrule
            \multicolumn{8}{c}{\textbf{\textit{LlaMa-2 7B With Retrieval}}} \\
            Direct RAG & 32.26 & 40.06 & 33.12 & 46.20 & 24.18 & 34.94 & 29.82 & 40.4 \\
            SFT RAG & 38.71 & 42.33 & \underline{36.58} & \underline{46.09} & \underline{25.59} & 35.15 & 33.64 & 41.19 \\
            GPT4 Rewriter + SFT RAG & \underline{42.22} & \underline{46.04} & 36.13 & 46.02 & 25.29 & \underline{35.38} & \underline{34.54} & \underline{42.49} \\
            ReAct~\citep{yao2023react} & 27.21 & 31.49 & 22.45 & 31.24 & 21.91 & 29.83 &  23.86 & 30.85 \\
            IRCoT~\citep{trivedi2023interleaving} & 9.22 &  17.93 & 13.52 & 25.94 & 17.42 & 27.13 & 13.39 & 23.67 \\
            % SKR\textsubscript{knn}~\citep{SKR} & 39.27 & 43.40 & 29.29 & 38.55 & 24.17 & 33.61 &   & \\
            SKR\textsubscript{knn}~\citep{SKR} & 36.04 & 39.59 & 35.41 & 44.75 & 23.63 & 33.44 &  31.68 & 39.26 \\
            \textbf{SmartRAG(ours)} & \textbf{44.32} & \textbf{47.60} & \textbf{37.89} & \textbf{47.76} & \textbf{26.60} & \textbf{36.42} & \textbf{36.27} & 43.93\\

            
            \bottomrule
        \end{tabular}
    }
    \caption{\label{tab:main} Overall experiment results on open-domain QA tasks. Bold numbers indicate the best performance among all methods in this model, and the underline indicates the second-best result.}
\end{table*}
% Cite加在后面 

%\subsection{Main Results}

%In the open-domain QA scenarios of our experiments, the answers generated after retrieval generally yield better results compared to direct answers. Therefore, to promote retrieval, we have set a relatively low retrieval threshold in Table \ref{tab:main} to encourage the retrieval process. Our SmartRAG demonstrates a substantial performance advantage over all methods in all three datasets, which demonstrates the effectiveness of our method within the RAG System. The observed improvement primarily stems from our framework's ability to optimize both the query rewrite and answer-from-observation tasks, particularly the query rewrite. Previous approaches were unable to optimize all tasks within an adaptive retrieval scenario using a single model. In contrast, SmartRAG effectively integrates the retrieval process with LLMs and the retrieval database itself, leading to retrieval behavior that more accurately reflects real-world scenarios. SmartRAG considers the current forms of generator LLMs and retrieval databases, which enables the generation of more target-aligned retrieval queries and provides more accurate responses based on the retrieved content.



We compare our proposed SmartRAG with all the baselines in Table~\ref{tab:main}. Following \citet{adaptiverag, selfrag}, we use two different types of base LLMs, \emph{i.e.} Flan-T5 large~\citep{chung2024scaling} and LlaMa2-7B~\citep{touvron2023llama}. \textbf{ICL} and \textbf{SFT} show the results without retrieval. the performance is obviously very poor, indicating that retrieving is necessary for these datasets. All the algorithms that has retrieve-related modules significantly increase the performance. By jointly optimizing all the related modules, our SmartRAG is able to outperform all the counterparts that uses separately optimized modules. This validates our argument that jointly optimization is necessary to make all the modules properly work together to achieve optimal performance. (Comment on CoT related algorithms)


\subsection{SmartRAG Knows When to Retrieve}



The first token of the action $\textbf{a}$ indicates whether to retrieve or not. In practice, the policy network outputs a Bernoulli distribution over $\{\Answer, \Query\}$, we can manually set up a threshold on the logit of \Answer to control the ratio of retrieval. Figure~\ref{fig:curve} shows the F1 score of SmartRAG with different thresholds. We compare SmartRAG with two baselines. The first one is SFT. Since it does not have any decision maker to decide whether to retrieve, it only has two states: full retrieve and no retrieve. The second baseline is SKR~\citep{wang2023self}, which trains a small module to decide whether to retrieve. The golden answer is provided by whether the answer generation module can produce the correct result. We can see that the results of SmartRAG is to the upper left side of the other methods, meaning that the SmartRAG can produce similar F1 score with less retrieval cost. On the PopQA dataset, SmartRAG even produces higher F1 score with less retrieval percentage comparing to SKR. To achieve this, SmartRAG should put more retrieval efforts on the scenarios when retrieval does brings benefit. In these scenarios, the base LLMs do not inherently know the correct answer but the knowledge is included in the database.

A deduction about the above arguments is that, the SmartRAG system should not retrieve anything if the database hardly contains any useful knowledge. This is indeed the case for Bing search engine on OpenBookQA, MedQA-cn and ARC-c datasets. We list the retrieval percentage and accuracy on these datasets in Table~\ref{tab:no_retrieval}. SFT and SFT RAG produce extremely close accuracy since the database contains very little knowledge on these datasets. The SKR method still produces a high retrieval percentage, which wastes the retrieval resources. Our SmartRAG is aware of the property of the database and learns not to retrieve in these cases.


% checkpoint 记录： full retrieval test 是/RL4LMs/rl4lm_exps/rl4lm_experiment_t5_base_ppo_full_three_v14/checkpoints/checkpoint_5
% large T5 checkpoint: /cpfs/user/gaojingsheng/AliA800/RL4LMs/rl4lm_exps/rl4lm_experiment_t5_large_ppo_v14/checkpoints/checkpoint_10

% 不同threshold的checkpoint是： 

% llama 7b是/cpfs/user/gaojingsheng/JapanA100/RL4LMs/rl4lm_exps/rl4lm_experiment_llama_ppo_full_three_v4/checkpoints/checkpoint_2

%To illustrate the effectiveness of our approach in the adaptive retrieval task, we conducted a comparative analysis with SFT RAG and SKR, focusing on the relationship between performance and retrieval percentage. The results are presented in Figure \ref{fig:curve}. The results clearly demonstrate that our reinforcement learning-based framework consistently outperforms both the SFT and previous adaptive retrieval methods across all different retrieval percentages. The observed improvements stem from the optimization of the decision to retrieve or not, as well as our framework's ability to simultaneously enhance the three previously mentioned RAG tasks: direct answer, query rewrite, and answer from observation. Additionally, it is evident that as the retrieval percentage increases, the effectiveness of our framework becomes more pronounced. This is because, at lower retrieval percentages, the gains primarily come from the direct answer task. Given that SFT has already been thoroughly optimized for direct answer, the room for further improvement in this area is limited. However, as the retrieval percentage increases, the decision-making regarding whether to retrieve or not becomes more significant, and the tasks of query rewrite and answer from observation also contribute to a substantial improvement in RAG's response quality. Consequently, the comparative gains over SFT become increasingly larger as the retrieval percentage rises.

% More pics.
% \myparagraph{Retrieval Threshold}

% 我们的方法可以找到一个更好的初态，同时我们还能滑threshold，所以我们在不同的database，不滑threshold
% 这张表要放state v2的结果
\begin{figure}[t]
    \centering
%    \begin{subfigure}[t]{0.32\textwidth}
%        \centering
%        \resizebox{\textwidth}{!}{
%        \includegraphics{pics/large_state/oracle_em_t5base_popqa.pdf}}
%    \end{subfigure}
%    \begin{subfigure}[t]{0.32\textwidth}
%        \centering
%        \resizebox{\textwidth}{!}{
%        \includegraphics{pics/large_state/oracle_em_t5base_ambignq.pdf}}
%    \end{subfigure}
%    \begin{subfigure}[t]{0.32\textwidth}
%        \centering
%        \resizebox{\textwidth}{!}{
%        \includegraphics{pics/large_state/oracle_em_t5base_hotpotqa.pdf}}
%    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
        \includegraphics{pics/large_state/oracle_f1_t5base_popqa.pdf}}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
        \includegraphics{pics/large_state/oracle_f1_t5base_ambignq.pdf}}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
        \includegraphics{pics/large_state/oracle_f1_t5base_hotpotqa.pdf}}
    \end{subfigure}
    \caption{\label{fig:curve}F1 Score of different retrieval percentage across three datasets on Flan-T5-large.}

\end{figure}
% 包括需要retrieval的，是指不检索回答不对，检索才能回答对的，
% 包括直接能回答对或者检索后都回答不对的
%\myparagraph{Results Analysis} To further investigate the decision-making performance of different methods on whether to retrieve, we defined a new metric call retrieval awareness, $\gR$. We categorized the instances where the model could not provide a correct answer directly into two types: those that requires retrieval, meaning those where the model cannot provide a correct answer without retrieval but can do so when retrieval is performed. $\gT$, and those that not need retrieval, including cases where the model can directly provide the correct answer or fails to answer correctly even after retrieval, $\gF$. As we adjust the retrieval threshold, both $\gT$ and $\gF$ retrieval ratios increase or decrease simultaneously. To enable a consistent comparison across different thresholds, we calculate the retrieval probability for each instance and then adjust the threshold so that the $\gF$ retrieval ratio is fixed at a certain value. At this fixed $\gF$ retrieval ratio, we compute the $\gT$ retrieval ratio. Under the same $\gF$ retrieval ratio, a higher $\gT$ retrieval ratio indicates better performance. The $\gR$ can be formulated as:

%\begin{equation}
%    \gR = \sum_{\evf=0}^{\evf=1} \evt / N
%\end{equation}

%where $\evf$ represents the retrieval ratio of $\gF$, and $\evt$ represents the retrieval ratio of $\gT$, N the sampling number of $\evf$. 

%The results of retrieval awareness $\gR$ is shown in Table \ref{tab:aware}, we can see that our method, due to its ability to recognize differences in the database, demonstrates the best decision-making performance, especially on the PopQA dataset, further validating the effectiveness of our framework.

% 
\begin{table}
    \centering
    \footnotesize
    % \setlength{\tabcolsep}{1.5mm}
    % \renewcommand{\arraystretch}{0.8} 
    \begin{tabular}{l|ccc|ccc}
    \toprule
    {\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{\textbf{\textit{Retrieval Percentage}}} & \multicolumn{3}{c}{\textbf{\textit{Accuracy}}} \\
     & OpenBookQA & MedQA-cn & ARC-c & OpenBookQA & MedQA-cn & ARC-c  \\ 
    \midrule
    SFT & 0.00 & 0.00 & 0.00 & 67.20 &  31.66 & 54.95 \\
    % SFT-S &  &    &   \\
    SFT RAG & 100 & 100 & 100 & 68.20 &  31.11 &  56.99\\
    \midrule
    SKR & 5.60 & 84.29 & 9.98 & 67.20 & 31.89 & 54.86 \\
    SmartRAG(Ours) & 0.00 & 0.00 & 0.00 & 66.60 & 33.31 & 55.72 \\ 
    % \midrule
    % \multicolumn{4}{c}{\textbf{\textit{Retrieval Percentage }}} \\
    % SKR & 5.60  & 84.29  &  9.98 \\
    % Ours &  0.00  &  0.00  & 0.00 \\
    \bottomrule
    \end{tabular}
    \caption{\label{tab:no_retrieval} Results of different one-choice questions on Flan-T5-large. All the methods produce similar accuracy since the database do not contain the useful answer. Our SmartRAG learns this property and learns not to retrieve.}
\end{table}



% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     Dataset & PopQA & AmbigNQ & HotpotQA \\ 
%     \midrule
%     SFT &  0.500  &  0.500   &   0.500  \\
%     SKR &  0.398  &  0.524 &  0.530 \\
%     Ours &  0.636  & 0.529  & 0.546  \\
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:aware} Retrieval awareness of different methods on three datasets of Flan-T5-large.}
    
% \end{table}

%\begin{table}
%    \centering
%    \footnotesize
%    % \setlength{\tabcolsep}{1.5mm}
%    \renewcommand{\arraystretch}{0.8} 
%    \begin{tabular}{lcccc}
%    \toprule
%    Dataset & PopQA & AmbigNQ & HotpotQA & Average \\ 
%    \midrule
%    SFT &  0.500  &  0.500   &   0.500  \\
%    % SKR &  0.398  &  0.524 &  0.530 \\
%    SKR &  0.499  &  0.514 &  0.547 \\
%    % Ours &  0.636  & 0.529  & 0.546  \\
%    PPO & 0.547 &  0.552  &  0.530  \\
%    \bottomrule
%    \end{tabular}
%    \caption{\label{tab:aware} Retrieval awareness of different methods on three datasets of Flan-T5-large.}    
%\end{table}

% 为了进一步研究不同的方法在是否检索这个问题上面的决策表现，我们对定义了一个新的metrics \gR。我们将模型不能直接回答对的数据分类两大类，检索后能够回答对的数据\gT和检索后仍然不能回答对的数据\gF。当我们移动检索的阈值时，\gT和\gF检索比例都会同时变大和变小。为了统一不同阈值下研究两者的对比，我们计算每条数据的检索概率，然后移动阈值让\gF检索比例为一个定值，在此定值下去计算\gT的检索比例。而在同一个\gF的检索比例下，\gT的检索比例应该越高越好。


% 横坐标是多少负样本被检索出来，纵坐标是正样本检索比例

% 同时把面积求出来

% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     Dataset & ours & SKR \\ 
%     \midrule
%     Direct Right  & 66.67 & 71.43  \\ % 56/84    &  60/84  \\ 
%     Retrieval False  & 85.06 & 64.94  \\  % 410/482  & 313/482  \\ 
%     Retrieval Right  &  87.76 & 63.27 \\ %  129/147  &   93/147 \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:transfer} Retrieval percentage of different data types on PopQA.}
% \end{table}

% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     Dataset & ours & SKR \\ 
%     \midrule
%     Direct Right  &  30.43 & 73.91 \\ % 7/23    &  17/23  \\ 
%     Retrieval False  &  20.78 & 91.57 \\ % 175/842  & 771/842  \\ 
%     Retrieval Right  &   33.33 & 95.56 \\ % 45/135  &   129/135\\ 
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:transfer} Retrieval percentage of different data types on AmbigNQ.}
% \end{table}

% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     Dataset & ours & SKR \\ 
%     \midrule
%     Direct Right  &  42.15 &  44.63 \\ % 51/121    &  54/121  \\ 
%     Retrieval False  &  57.38 & 77.75 \\ % 459/800  & 622/800  \\ 
%     Retrieval Right  &   58.23 & 77.22 \\ % 46/79  &   61/79\\ 
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:transfer} Retrieval percentage of different data types on HotpotQA.}
% \end{table}

% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     Dataset & ours & SKR \\ 
%     \midrule
%     Direct Right  & 60.80 & 46.23  \\ % 121/199    &  92/199 \\ 
%     Retrieval False  & 58.00 & 80.79  \\  % 221/381  &  307/380 \\ 
%     Retrieval Right  &  59.09 & 71.21 \\ %  78/132  &   94/132 \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:transfer} Retrieval percentage of different data types on PopQA.}
% \end{table}

% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     Dataset & ours & SKR \\ 
%     \midrule
%     Direct Right  &  30.43 & 73.91 \\ % 7/23    &  17/23  \\ 
%     Retrieval False  &  20.78 & 91.57 \\ % 175/842  & 771/842  \\ 
%     Retrieval Right  &   33.33 & 95.56 \\ % 45/135  &   129/135\\ 
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:transfer} Retrieval percentage of different data types on AmbigNQ.}
% \end{table}

% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     Dataset & ours & SKR \\ 
%     \midrule
%     Direct Right  &  42.15 &  44.63 \\ % 51/121    &  54/121  \\ 
%     Retrieval False  &  57.38 & 77.75 \\ % 459/800  & 622/800  \\ 
%     Retrieval Right  &   58.23 & 77.22 \\ % 46/79  &   61/79\\ 
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:transfer} Retrieval percentage of different data types on HotpotQA.}
% \end{table}

\subsection{SmartRAG Knows What to Retrieve}

Once SmartRAG decides to retrieve the database, the next question is what to retrieve. Directly searching for the original question produces suboptimal performance, as Table~\ref{tab:main} demonstrates. In Table~\ref{tab:query_rewrite}, we further showcase that our SmartRAG can produce better search query and thus improving the final answer accuracy. In the first question \textit{Who was the producer of 9}, directly searching the question cannot provide any useful information. As a result, the model generates an answer based on its own knowledge and gives the wrong answer. The rewritten query \textit{Who produced the movie 9} is aware of that \textit{9} is a name of a film and explicitly uses the term \textit{movie 9}. With this modification, the retrieved result is more related and contains the correct answer, which is then output by the answer generator in the next step.

\begin{table*}[t!]
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{2pt}
\footnotesize
\centering
\begin{tabular}{p{13cm}}%|ccccccc}
\toprule

{\bf Question 1: } Who was the producer of 9? \\
{\bf Golden Answer:} Shane Acker \\
{\bf Observation with original question: }5 Things to Know About THE9, China 2019s New Pop Idol Group: Predicting the shelf-life of a pop act is never straightforward, but it will be interesting to see just how long THE9 stick around given the rapid demise of boyband Nine Percent, who were spawned by 2018-2019s Idol Producer. \\
{\bf Output: }\Answer \color{red}{Tim Burton}\\
\midrule
{\bf Rewritten Query: }Who produced the movie 9? \\
{\bf Observation with rewritten query: }9 (2009) - IMDb: Shane Acker first made 9 (2009) as a ten minute short film while he was still at UCLA. It was nominated for Best Animated Short at the Oscars, and although it didn't win, Acker was offered the chance to expand it into a feature film. \\
{\bf Output: } \Answer \color{green}{Shane Acker} \\ 
\midrule
\midrule

{\bf Question 2: } When was the contruction of the makkah royal clock tower hotel started? \\
{\bf Golden Answer: } 2004\\
{\bf Observation with original question: } Ryugyong Hotel: Ryugyong Hotel was designed by North Korean firm Baikdoosan Architects and Engineers, which is also the contractor of the project before 1992, the firm had built the building to its full height before the construction suspended in 1992. ... However, considering Ryugyong Hotel is 112 meters shorter than Willis Tower, 360,000 square meters is still ... \\
{\bf Output: }\Answer \color{red}{1992} \\
\midrule
{\bf Rewritten Query: }Start date of construction for the Makkah Royal Clock Tower Hotel \\
{\bf Observation with rewritten query:  }Makkah Royal Clock Tower, Saudi Arabia - World Construction Network: The Makkah Royal Clock Tower complex, also known as the Abraj Al-Bait Towers, located near Masjid al Haram in Mecca, Saudi Arabia, is a mixed residential and hotel complex. Construction on the complex was started in 2004 and finished in 2012. \\
{\bf Output: } \Answer \color{green}{2004} \\ 
\midrule
\midrule

{\bf Question 3: }My Babysitter's a Vampire was created by Fresh TV, who also created which Canadian animated sitcom which premiered in Canada on November 7, 2004 on Teletoon? \\
{\bf Golden Answer: } 6teen\\
{\bf Observation with original question: } My Babysitter's a Vampire (TV Series 2011\u20132012) - IMDb: My Babysitter's a Vampire: Created by Jennifer Pertsch, Tom McGillis. With Matthew Knight, Vanessa Morgan, Atticus Mitchell, Cameron Kennedy. Ethan Morgan, his half-vampire babysitter and pals battle against creatures from their nightmares. \\
{\bf Output: }\Answer \color{red}{Total Drama} \\
\midrule
{\bf Rewritten Query: }Which Canadian animated sitcom, premiered on Teletoon on November 7, 2004, was created by Fresh TV and also created My Babysitter's a Vampire?  \\
{\bf Observation with rewritten query: }6Teen Wiki: 6teen, originally known as The Mall, is a Canadian animated teen sitcom created by Tom McGillis and Jennifer Pertsch. It first aired on Teletoon on November 7, 2004 until February 11, 2010. It is set in the fictional Galleria Mall and follows an ensemble cast of six sixteen-year-old friends as... \\
{\bf Output: } \Answer \color{green}{6teen} \\ 

\bottomrule
\end{tabular}
 
\caption{Improvement of query rewrite in comparison to origin question.}\label{tab:query_rewrite}

\end{table*}



To further validate that the query rewrite module does play its role in enhancing the overall performance, we replace all the retrieving queries in our SmartRAG pipeline with the original question. The evaluation result is shown in Table~\ref{tab:query}. Using the original question to retrieve does degrade the performance on all the datasets over all the metrics.

\begin{table}[t]
    \centering
    \hspace{0.05\textwidth} % 调整minipage之间的距离
    \begin{minipage}[b]{0.4\textwidth}
        \centering
        \footnotesize
        \setlength{\tabcolsep}{1.5mm}
        \begin{tabular}{llccc}
        \toprule
        Search & DataSet & EM  & F1  & hit \\ 
        \midrule
    
        \multirow{3}{*}{Question} & PopQA &  39.31 &  43.79 &  47.97 \\ 
        & AmbigNQ & 32.48   &  41.49 &  48.81 \\ % 73.5
        & HotpotQA & 24.33  &  34.21   &  32.03  \\ 
        \midrule
        \multirow{3}{*}{SmartRAG} & PopQA  &  41.66  &  45.95  &  51.47 \\ 
        & AmbigNQ  &  32.68  &  42.56  &  50.88\\
        & HotpotQA &  26.08 &  36.26  &  34.52 \\ 
        
        \bottomrule
        \end{tabular}
        \caption{\label{tab:query} Replace search query with original question.}
    \end{minipage}%
\end{table}



\subsection{Analysis} % Mainly T5?

\myparagraph{Different Initial State} For a reinforcement learning algorithm, an optimal initial state facilitates the model's exploration of a more advantageous solution space. In the previous SFT process, the model's initial state for deciding whether to retrieve information for each query is random. However, by incorporating the model's inference results into the training set as guidance, each data point in SFT is assigned a specific retrieval initial state. This allows the model to acquire certain decision-making capabilities by the end of SFT. This approach closely aligns with SKR's method of classification based on self-knowledge. Thus, we conducted a new round of SFT to investigate the impact of different initial states on the reinforcement learning process, with the training setup detailed in the Appendix. The results of SFT with two distinct initial states, along with post-PPO results, are illustrated in the Figure. As shown, with the new initial state, the model demonstrates some decision-making ability even during SFT. Under this enhanced decision-making capability, PPO further refines the decisions, leading to superior outcomes. When the retrieval percentage is 0 or 100, the results across different states are nearly identical, which supports our conclusion that a better decision-making initial state helps reinforcement learning explore more optimal decision points, while its influence on direct answer and full retrieval states is minimal.



\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.63\textwidth} % 图的minipage
        \centering
        \begin{subfigure}[t]{0.49\textwidth}
            \centering
            \resizebox{\textwidth}{!}{
            \includegraphics{pics/stateV2/oracle_em_t5base_popqa.pdf}}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.49\textwidth}
            \centering
            \resizebox{\textwidth}{!}{
            \includegraphics{pics/stateV2/oracle_f1_t5base_popqa.pdf}}
        \end{subfigure}
        \caption{Influence of different warm up state.}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.35\textwidth} % 表的minipage
        \centering
        \footnotesize
        \setlength{\tabcolsep}{1mm}
        \begin{tabular}{lccc}
        \toprule
        Method & EM & F1  &  Awareness\\ 
        \midrule
        SFT  &  47.72 &  56.99  & 0.500 \\ 
        SKR  &  37.51 &  45.35  &  0.523 \\ 
        Ours &  48.87 &  59.17  & 0.552 \\ 
        \bottomrule
        \end{tabular}
        \caption{\label{tab:transfer} Dataset Transfer on TriviaQA of Flan-T5-large.}
    \end{minipage}
\end{figure}
% How to describe? 


% Weaker database will get lower retrieval percentage and worse performance.
% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     DataSet & EM  & F1  \\ 
%     \midrule
%     PopQA  &  34.36  &  38.43  \\ 
%     AmbigNQ  &  17.01  &  25.05  \\ 
%     HotpotQA &   21.32 &  30.09  \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:query} Results of Contriever different database.}
% \end{table}
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
        \includegraphics{pics/Num/oracle_em_t5base_popqa.pdf}}
        % \caption{Exact match of different retrieval number K.}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
        \includegraphics{pics/Num/oracle_f1_t5base_popqa.pdf}}
        %\caption{F1 score of different retrieval number K.}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
        \includegraphics{pics/Num/threshold.pdf}}
        % \caption{Relationship between threshold and retrieval percentage on Flan-T5-large.}
    \end{subfigure}
    \caption{Exact Match, F1 Score and Retrieval Threshold of different retrieval number K on Flan-T5-large.}
\end{figure}

\myparagraph{Retrieval Number K} In the retrieval-augmented framework, the number of retrieved texts also influences the model's performance. Generally, when the number of retrieved documents is not large, an increase in the number of retrieved documents leads to greater gains for the model. This is because when the retrieved information falls within the model's capacity to process, a larger set of documents is more likely to contain useful information. Therefore, we investigated the model's performance when the retrieval size is K=1 and K=4. When K=4, it represents a retrieval of more documents and a stronger retrieval capacity, allowing us to explore the impact of varying value database on our method's training results. The results, as shown in the figure, indicate that retrieving more documents leads to better performance. The figure also illustrates the relationship between the retrieval ratio and the threshold under different retrieval intensities. It is evident that when the retrieval database is more likely to contain relevant information, our method can demonstrate better awareness of the database, which in turn drives the model to rely more on retrieval. This aligns with real-world scenarios, where higher retrieval efficiency should increase the likelihood of the model engaging in retrieval, and vice versa. In contrast, the previous adaptive retrieval method was unable to recognize the impact of different databases.

% Simply set to 1, what conclusion?

% Better retrieval num means better retrieval performance and large percentage. (in fact, it is not robust due to threshold move)

% 不同的初态去观察检索比例，如果仍然观察不到就直接说结果更好
% 设计一个更好的指标

\myparagraph{Dataset Transfer} Given that our framework emphasizes the importance of making the model aware of the retrieval database, we tested the model trained with our framework on the TriviaQA dataset in a data migration scenario. The goal was to explore whether this database awareness could transfer to other datasets. We categorized the TriviaQA test set into three types: the first type includes questions that can be answered correctly after supervised fine-tuning (SFT) without retrieval; the second type consists of questions that can only be answered correctly after retrieval; and the third type contains questions that cannot be answered correctly even after retrieval. Ideally, the model should avoid retrieval for the first and third types and opt for retrieval only for the second type. We tested the retrieval proportion for these three data types, and the results are presented in Table \ref{tab:transfer}. It is evident that the second type of data maintains the highest retrieval percentage, while the first type has a relatively lower retrieval percentage. This indicates that in transfer testing scenarios, our model retains a certain level of database awareness.


% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     Data Type & Retrieval Percentage(\%) & SKR  & SFT\\ 
%     \midrule
%     Direct Right  &   26.67    & 73.33 & 50  \\ 
%     Retrieval False  &   37.29  & 84.63  & 50 \\ 
%     Retrieval Right  &   41.85   &  85.30 & 50 \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:transfer} Dataset Transfer on TriviaQA.}
% \end{table}




\myparagraph{Query Rewrite Improvement} A key aspect of our framework is its ability to optimize the query. We conducted a quantitative analysis of the extent to which our framework enhances the query rewrite task. Specifically, we evaluated our model after PPO by setting a threshold to achieve a full retrieval state. During each retrieval, we replaced the generated query with the original question to compare the advantages of our generated query over the original one. The results, presented in Table \ref{tab:query}, indicate that our method significantly improves query rewriting across almost all datasets, with the exception of the F1 score on AmbigNQ. This suggests that reinforcement learning can effectively modify the retrieval query to better understand the database, thereby enhancing overall performance by retrieving more relevant content.

% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     DataSet & EM  & F1  & hit \\ 
%     \midrule
%     PopQA-b  &  33.66  &  37.87 &   \\ 
%     AmbigNQ-b  &  18.31  &  27.71  & \\ % 64.4
%     HotpotQA-b &  18.24 &  27.26 &  \\ 
%     \midrule
%     PopQA-q &   31.84  &  35.46  & \\ 
%     AmbigNQ-q &   18.18  &  28.17   & \\ % 73.5
%     HotpotQA-q &  17.70   &   26.89  &  \\ 
    
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:query} Replace search query with original question.}
% \end{table}


% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     DataSet & EM  & F1  & hit \\ 
%     \midrule
%     PopQA-b  &  35.48  &  39.73  &  51.47 \\ 
%     AmbigNQ-b  &  20.53  &  30.94  &  50.88\\ % 64.4
%     HotpotQA-b &  22.17 & 31.72 &  34.52 \\ 
%     \midrule
%     PopQA-q &  32.89 &  37.30 &  47.97 \\ 
%     AmbigNQ-q &  19.58   &  29.59 &  48.81 \\ % 73.5
%     HotpotQA-q &  20.64  &  29.95   &  32.03  \\ 
    
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:query} Replace search query with original question.}
% \end{table}

% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{llccc}
%     \toprule
%     Search & DataSet & EM  & F1  & hit \\ 
%     \midrule

%     \multirow{3}{*}{Question} & PopQA &  39.31 &  43.79 &  47.97 \\ 
%     & AmbigNQ & 32.48   &  41.49 &  48.81 \\ % 73.5
%     & HotpotQA & 24.33  &  34.21   &  32.03  \\ 

%     \midrule

%     \multirow{3}{*}{Ours} & PopQA  &  41.66  &  45.95  &  51.47 \\ 
%     & AmbigNQ  &  32.68  &  42.56  &  50.88\\
%     & HotpotQA &  26.08 &  36.26  &  34.52 \\ 
    
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:query} Replace search query with original question.}
% \end{table}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.48\textwidth}
%         \centering
%         \resizebox{\textwidth}{!}{
%         \includegraphics{pics/f1_score_t5base.png}}
%         \caption{F1 Score of Flan-T5 base during Training.}
%         \label{fig:em_left}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.48\textwidth}
%         \centering
%         \resizebox{\textwidth}{!}{
%         \includegraphics{pics/f1_score_llama.png}}
%         \caption{F1 Score of LlaMa-7B base during Training.}
%         \label{fig:f1_right}
%     \end{subfigure}
%     % \caption{Pareto Curve.}
%     \label{fig:em}
% \end{figure}

%\begin{table}[t]
%    \centering
%    \hspace{0.05\textwidth} % 调整minipage之间的距离
%    \begin{minipage}[b]{0.41\textwidth}
%        \centering
%        \footnotesize
%        \setlength{\tabcolsep}{1.5mm}
%        \begin{tabular}{llccc}
%        \toprule
%        Search & DataSet & EM  & F1  & hit \\ 
%        \midrule
    
%        \multirow{3}{*}{Question} & PopQA &  39.31 &  43.79 &  47.97 \\ 
%        & AmbigNQ & 32.48   &  41.49 &  48.81 \\ % 73.5
%        & HotpotQA & 24.33  &  34.21   &  32.03  \\ 
%        \midrule
%        \multirow{3}{*}{Ours} & PopQA  &  41.66  &  45.95  &  51.47 \\ 
%        & AmbigNQ  &  32.68  &  42.56  &  50.88\\
%        & HotpotQA &  26.08 &  36.26  &  34.52 \\ 
        
%        \bottomrule
%        \end{tabular}
%        \caption{\label{tab:query} Replace search query with original question.}
%        \end{minipage}%
%    \hfill
%    \begin{minipage}[b]{0.45\textwidth}
%        \centering
%        \includegraphics[width=0.9\textwidth, height=0.54\textwidth]{pics/Size.pdf}
%        \caption{Retrieval awareness of different model sizes.}
%    \end{minipage}
%\end{table}

\myparagraph{Model Size} To further explore the training performance of models of different sizes within our framework, we examined the Flan-T5 series with various model sizes. By observing how different model sizes affect the retrieval awareness metric, we analyzed the models' decision-making capabilities regarding whether retrieval is necessary. As shown in the results (refer to the figure), we can see that as the model size increases, retrieval awareness also improves significantly.


%\myparagraph{Multi-choice QA} The scores on one-choice QA are presented in Table \ref{tab:selection}. We observe that our RAG provides only a modest improvement in the overall QA accuracy, indicating that RAG struggles to retrieve useful information in these challenging scenarios. However, our training framework can easily recognize this limitation, ultimately opting not to retrieve during training. In contrast, previous classifier-based methods still maintain a high retrieval rate, further demonstrating the superiority of our joint training approach with the database. Additionally, since our method optimizes direct answers on top of SFT, it results in a significant improvement in the quality of direct answers.


% It can be observed that our method is still able to enhance the model's performance across different retrieval percentages.

% OpenBook RAG is useless, ours learns all not retrieve, SKR retrieval percentage is large

% MMLU cannot achieve a proper training, debug find due to max length, query too long
% \begin{table}
%     \centering
%     \footnotesize
%     % \setlength{\tabcolsep}{1.5mm}
%     \begin{tabular}{lccc}
%     \toprule
%     \multicolumn{4}{c}{\textbf{\textit{Influence of Retrieval}}} \\
%     Method & OpenBookQA & MedQA-en & ARC-c  \\ 
%     SFT & 32.60  &  24.04  &  28.41 \\
%     % SFT-S &  &    &   \\
%     SFT RAG &  28.00  &  23.72  & 28.33 \\
%     SKR &  &  & \\
%     Ours & 61.80 &  30.72 & 56.57 \\
%     \midrule
%     \multicolumn{4}{c}{\textbf{\textit{Retrieval Percentage of different Method}}} \\
%     SKR &  &  &   \\
%     Ours &  0 &  0  &  0 \\
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:selection} Results of different multi-choice questions.}
% \end{table}
% 




% \begin{table}
%     \centering
%     \footnotesize
%     \begin{tabular}{lccc}
%     \toprule
%     Method & PopQA & AmbigNQ & HotpotQA  \\ 
%     \midrule
%     SFT-base &  0.546 &  0.546  & 0.528 \\
%     % SFT-base &  0.515 &  0.503  & 0.499 \\
%     PPO-base &  0.549 &  0.586  & 0.559 \\
%     % PPO-base &  0.549 &  0.566  & 0.514 \\
%     SFT-large &  0.377 &  0.495  & 0.570\\
%     PPO-large &  0.636 &  0.529  & 0.546 \\
%     SFT-xl &  0.579 &  0.523  & 0.472  \\
%     PPO-xl &   &    & \\
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:awareness} Retrieval Awareness.}
% \end{table}




% \begin{table}
%     \centering
%     \footnotesize
%     \begin{tabular}{lccc}
%     \toprule
%     Method & PopQA & AmbigNQ & HotpotQA  \\ 
%     \midrule
%     SFT-base &  0.503  &  0.499  &   0.496   \\
%     PPO-base &  0.558 &  0.539  &  0.522    \\
%     SFT-large & 0.547  &  0.539  &  0.511 \\
%     PPO-large & 0.547 &  0.552  &  0.530  \\
%     SFT-xl &  0.565  &  0.531  &  0.526  \\
%     PPO-xl &  0.593  &  0.542  &  0.531  \\
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:awareness} Retrieval Awareness.}
% \end{table}


% 不同大小模型的决策能力

% How to show model size influence? Large Size is better?
% 很难得到模型越大能力越强

% 纵坐标是决策面积，按道理越大就越强

% 验证不同database强度的影响


% \myparagraph{Improvement of Three Tasks}


% Except This 

% Training Results and Training Reward


% Concern: Limited Improvement on two tasks?

% \myparagraph{Improvement of Direct Answer}


% \myparagraph{Improvement of Query Write}


% \myparagraph{Improvement of Answer from Observation}

